Efficient computation of the volume of a polytope in high-dimensions using Piecewise Deterministic Markov Processes

Computing the volume of a polytope in high dimensions is computationally challenging but has wide applications. Current state-of-the-art algorithms to compute such volumes rely on efficient sampling of a Gaussian distribution restricted to the polytope, using e.g. Hamiltonian Monte Carlo. We present a new sampling strategy that uses a Piecewise Deterministic Markov Process. Like Hamiltonian Monte Carlo, this new method involves simulating trajectories of a non-reversible process and inherits similar good mixing properties. However, importantly, the process can be simulated more easily due to its piecewise linear trajectories - and this leads to a reduction of the computational cost by a factor of the dimension of the space. Our experiments indicate that our method is numerically robust and is one order of magnitude faster (or better) than existing methods using Hamiltonian Monte Carlo. On a single core processor, we report computational time of a few minutes up to dimension 500.

==> fig-pdm-all-v1/batch-aggregated-misc.tex <==
20 & PDM-N10**5 & cube & 50 & NA & 1.000E+05 &  5.231E-01 &  NA & NA & NA & NA & NA & NA & 3.966E+00 &  7.503E-02 \\
20 & PDM-N10**6 & cube & 50 & NA & 1.000E+06 &  6.048E-01 &  NA & NA & NA & NA & NA & NA & 4.210E+01 &  5.739E-01 \\
\hdashline
20 & PDM-N10**5 & cube & 70 & NA & 1.000E+05 &  6.708E-01 &  NA & NA & NA & NA & NA & NA & 7.902E+00 &  2.531E+00 \\
20 & PDM-N10**6 & cube & 70 & NA & 1.000E+06 &  8.256E-01 &  NA & NA & NA & NA & NA & NA & 6.767E+01 &  2.002E+00 \\
\hdashline
20 & PDM-N10**5 & cube & 100 & NA & 1.000E+05 &  7.327E-01 &  NA & NA & NA & NA & NA & NA & 1.505E+01 &  4.508E-01 \\
20 & PDM-N10**6 & cube & 100 & NA & 1.000E+06 &  7.452E-01 &  NA & NA & NA & NA & NA & NA & 1.262E+02 &  2.604E+00 \\
\hdashline
20 & PDM-N10**5 & cube & 500 & NA & 9.999E+04 &  1.861E+00 &  NA & NA & NA & NA & NA & NA & 1.150E+03 &  6.112E+01 \\
20 & PDM-N10**6 & cube & 500 & NA & 1.000E+06 &  1.410E+00 &  NA & NA & NA & NA & NA & NA & 6.317E+03 &  3.269E+02 \\
\hline
20 & PDM-N10**5 & isotropic-$\Delta$ & 50 & NA & 1.000E+05 &  6.156E-01 &  NA & NA & NA & NA & NA & NA & 3.560E+00 &  8.623E-02 \\
20 & PDM-N10**6 & isotropic-$\Delta$ & 50 & NA & 1.000E+06 &  1.196E+00 &  NA & NA & NA & NA & NA & NA & 2.835E+01 &  3.105E-01 \\
\hdashline
20 & PDM-N10**5 & isotropic-$\Delta$ & 70 & NA & 9.999E+04 &  8.256E-01 &  NA & NA & NA & NA & NA & NA & 6.631E+00 &  1.186E-01 \\
20 & PDM-N10**6 & isotropic-$\Delta$ & 70 & NA & 1.000E+06 &  1.170E+00 &  NA & NA & NA & NA & NA & NA & 5.144E+01 &  6.674E-01 \\
\hdashline
20 & PDM-N10**5 & isotropic-$\Delta$ & 100 & NA & 9.999E+04 &  1.348E+00 &  NA & NA & NA & NA & NA & NA & 1.330E+01 &  3.103E-01 \\
20 & PDM-N10**6 & isotropic-$\Delta$ & 100 & NA & 1.000E+06 &  1.410E+00 &  NA & NA & NA & NA & NA & NA & 9.655E+01 &  1.091E+00 \\
\hdashline
20 & PDM-N10**5 & isotropic-$\Delta$ & 500 & NA & 9.998E+04 &  1.895E+00 &  NA & NA & NA & NA & NA & NA & 7.220E+02 &  2.991E+01 \\
20 & PDM-N10**6 & isotropic-$\Delta$ & 500 & NA & 1.000E+06 &  2.526E+00 &  NA & NA & NA & NA & NA & NA & 2.867E+03 &  7.791E+01 \\
\hline
20 & PDM-N10**5 & standard-$\Delta$ & 50 & NA & 1.000E+05 &  1.070E+00 &  NA & NA & NA & NA & NA & NA & 3.648E+00 &  9.834E-02 \\
20 & PDM-N10**6 & standard-$\Delta$ & 50 & NA & 1.000E+06 &  7.164E-01 &  NA & NA & NA & NA & NA & NA & 2.873E+01 &  2.845E-01 \\
\hdashline
20 & PDM-N10**5 & standard-$\Delta$ & 70 & NA & 9.999E+04 &  1.170E+00 &  NA & NA & NA & NA & NA & NA & 6.804E+00 &  1.694E-01 \\
20 & PDM-N10**6 & standard-$\Delta$ & 70 & NA & 1.000E+06 &  1.119E+00 &  NA & NA & NA & NA & NA & NA & 5.174E+01 &  4.734E-01 \\
\hdashline
20 & PDM-N10**5 & standard-$\Delta$ & 100 & NA & 9.999E+04 &  1.251E+00 &  NA & NA & NA & NA & NA & NA & 1.343E+01 &  2.695E-01 \\
20 & PDM-N10**6 & standard-$\Delta$ & 100 & NA & 1.000E+06 &  1.226E+00 &  NA & NA & NA & NA & NA & NA & 9.630E+01 &  1.102E+00 \\
\hdashline
20 & PDM-N10**5 & standard-$\Delta$ & 500 & NA & 9.998E+04 &  2.059E+00 &  NA & NA & NA & NA & NA & NA & 8.788E+02 &  5.198E+01 \\
20 & PDM-N10**6 & standard-$\Delta$ & 500 & NA & 1.000E+06 &  1.814E+00 &  NA & NA & NA & NA & NA & NA & 3.136E+03 &  5.033E+01 \\


==> fig-pdm-all-v1/batch-aggregated-volumes.tex <==
20 & PDM-N10**5 & cube & 50 & NA &1.126e+15 & 1.061e+15 & 1.173e+15 & 1.127e+15 & 3.569e+13 &  2.398E-02 &  1.920E-02 \\
20 & PDM-N10**6 & cube & 50 & NA &1.126e+15 & 1.062e+15 & 1.207e+15 & 1.148e+15 & 4.049e+13 &  2.836E-02 &  1.657E-02 \\
\hdashline
20 & PDM-N10**5 & cube & 70 & NA &1.181e+21 & 1.067e+21 & 1.272e+21 & 1.162e+21 & 5.594e+19 &  4.315E-02 &  2.919E-02 \\
20 & PDM-N10**6 & cube & 70 & NA &1.181e+21 & 1.069e+21 & 1.217e+21 & 1.192e+21 & 3.366e+19 &  1.379E-02 &  2.045E-02 \\
\hdashline
20 & PDM-N10**5 & cube & 100 & NA &1.268e+30 & 1.128e+30 & 1.439e+30 & 1.269e+30 & 8.047e+28 &  3.992E-02 &  3.991E-02 \\
20 & PDM-N10**6 & cube & 100 & NA &1.268e+30 & 1.172e+30 & 1.388e+30 & 1.256e+30 & 4.818e+28 &  2.348E-02 &  2.438E-02 \\
\hdashline
20 & PDM-N10**5 & cube & 500 & NA &3.273e+150 & 1.668e+150 & 5.659e+150 & 2.77e+150 & 1.085e+150 &  3.139E-01 &  1.777E-01 \\
20 & PDM-N10**6 & cube & 500 & NA &3.273e+150 & 2.311e+150 & 4.208e+150 & 3.215e+150 & 4.503e+149 &  8.394E-02 &  8.715E-02 \\
\hline
20 & PDM-N10**5 & isotropic-$\Delta$ & 50 & NA &3.421e+21 & 3.107e+21 & 3.92e+21 & 3.383e+21 & 2.124e+20 &  3.689E-02 &  3.885E-02 \\
20 & PDM-N10**6 & isotropic-$\Delta$ & 50 & NA &3.421e+21 & 3.285e+21 & 3.768e+21 & 3.441e+21 & 9.746e+19 &  1.314E-02 &  2.125E-02 \\
\hdashline
20 & PDM-N10**5 & isotropic-$\Delta$ & 70 & NA &1.658e+30 & 1.346e+30 & 1.976e+30 & 1.637e+30 & 1.49e+29 &  4.635E-02 &  6.144E-02 \\
20 & PDM-N10**6 & isotropic-$\Delta$ & 70 & NA &1.658e+30 & 1.548e+30 & 1.78e+30 & 1.64e+30 & 6.341e+28 &  3.127E-02 &  2.209E-02 \\
\hdashline
20 & PDM-N10**5 & isotropic-$\Delta$ & 100 & NA &1.771e+43 & 1.423e+43 & 2.073e+43 & 1.724e+43 & 2.057e+42 &  9.950E-02 &  5.106E-02 \\
20 & PDM-N10**6 & isotropic-$\Delta$ & 100 & NA &1.771e+43 & 1.53e+43 & 1.865e+43 & 1.759e+43 & 7.592e+41 &  2.608E-02 &  2.889E-02 \\
\hdashline
20 & PDM-N10**5 & isotropic-$\Delta$ & 500 & NA &9.235e+216 & 1.811e+216 & 1.33e+217 & 5.351e+216 & 3.312e+216 &  4.402E-01 &  2.601E-01 \\
20 & PDM-N10**6 & isotropic-$\Delta$ & 500 & NA &9.235e+216 & 6.724e+216 & 1.677e+217 & 8.775e+216 & 2.431e+216 &  1.690E-01 &  1.761E-01 \\
\hline
20 & PDM-N10**5 & standard-$\Delta$ & 50 & NA &3.288e-65 & 2.891e-65 & 3.612e-65 & 3.255e-65 & 2.356e-66 &  6.389E-02 &  3.704E-02 \\
20 & PDM-N10**6 & standard-$\Delta$ & 50 & NA &3.288e-65 & 3.148e-65 & 3.522e-65 & 3.284e-65 & 9.439e-67 &  1.742E-02 &  1.827E-02 \\
\hdashline
20 & PDM-N10**5 & standard-$\Delta$ & 70 & NA &8.348e-101 & 7.202e-101 & 9.817e-101 & 8.063e-101 & 7.353e-102 &  8.987E-02 &  4.940E-02 \\
20 & PDM-N10**6 & standard-$\Delta$ & 70 & NA &8.348e-101 & 8.048e-101 & 9.487e-101 & 8.472e-101 & 3.885e-102 &  3.017E-02 &  3.394E-02 \\
\hdashline
20 & PDM-N10**5 & standard-$\Delta$ & 100 & NA &1.072e-158 & 7.569e-159 & 1.369e-158 & 1.045e-158 & 1.452e-159 &  1.140E-01 &  7.437E-02 \\
20 & PDM-N10**6 & standard-$\Delta$ & 100 & NA &1.072e-158 & 9.994e-159 & 1.187e-158 & 1.113e-158 & 4.951e-160 &  4.255E-02 &  2.928E-02 \\
\hdashline
20 & PDM-N10**5 & standard-$\Delta$ & 500 & NA &8.196e-1135 & 9.322e-1134 & 1.04e-1132 & 2.339e-1133 & 2.507e-1133 &  2.753E+01 &  3.059E+01 \\
20 & PDM-N10**6 & standard-$\Delta$ & 500 & NA &8.196e-1135 & 1.615e-1133 & 5.068e-1133 & 3.277e-1133 & 8.501e-1134 &  3.899E+01 &  1.037E+01 \\


==> fig-pdm-all-v2/batch-aggregated-misc.tex <==
50 & PDMP-N10**5 & cube & 50 & NA & 5.468E+01 &  1.501E+00 & 0 &0 & 4.025E+00 &  8.019E-02 \\
50 & PDMP-N10**6 & cube & 50 & NA & 5.463E+01 &  1.248E+00 & 0 &0 & 3.583E+01 &  7.040E-01 \\
\hdashline
50 & PDMP-N10**5 & cube & 70 & NA & 7.627E+01 &  1.893E+00 & 0 &0 & 7.794E+00 &  1.817E-01 \\
50 & PDMP-N10**6 & cube & 70 & NA & 7.603E+01 &  2.271E+00 & 0 &0 & 6.784E+01 &  1.622E+00 \\
\hdashline
50 & PDMP-N10**5 & cube & 100 & NA & 1.084E+02 &  3.456E+00 & 0 &0 & 1.506E+01 &  4.787E-01 \\
50 & PDMP-N10**6 & cube & 100 & NA & 1.094E+02 &  3.739E+00 & 0 &0 & 1.261E+02 &  3.464E+00 \\
\hdashline
50 & PDMP-N10**5 & cube & 500 & NA & 5.187E+02 &  5.499E+00 & 0 &0 & 1.127E+03 &  6.796E+01 \\
50 & PDMP-N10**6 & cube & 500 & NA & 5.155E+02 &  4.751E+00 & 0 &0 & 6.595E+03 &  6.420E+02 \\
25 & PDMP-N10**7 & cube & 500 & NA & 5.123E+02 &  5.283E+00 & 0 &0 & 5.729E+04 &  1.107E+04 \\
\hline
50 & PDMP-N10**5 & isotropic-$\Delta$ & 50 & NA & 5.425E+01 &  5.376E-01 & 0 &0 & 3.712E+00 &  8.565E-02 \\
50 & PDMP-N10**6 & isotropic-$\Delta$ & 50 & NA & 5.320E+01 &  5.586E-01 & 0 &0 & 2.877E+01 &  4.387E-01 \\
\hdashline
50 & PDMP-N10**5 & isotropic-$\Delta$ & 70 & NA & 7.517E+01 &  8.637E-01 & 0 &0 & 6.690E+00 &  1.574E-01 \\
50 & PDMP-N10**6 & isotropic-$\Delta$ & 70 & NA & 7.367E+01 &  9.365E-01 & 0 &0 & 5.141E+01 &  5.792E-01 \\
\hdashline
50 & PDMP-N10**5 & isotropic-$\Delta$ & 100 & NA & 1.070E+02 &  1.309E+00 & 0 &0 & 1.368E+01 &  3.791E-01 \\
50 & PDMP-N10**6 & isotropic-$\Delta$ & 100 & NA & 1.047E+02 &  1.054E+00 & 0 &0 & 9.637E+01 &  1.424E+00 \\
\hdashline
50 & PDMP-N10**5 & isotropic-$\Delta$ & 500 & NA & 5.240E+02 &  3.540E+00 & 0 &0 & 7.503E+02 &  4.174E+01 \\
50 & PDMP-N10**6 & isotropic-$\Delta$ & 500 & NA & 5.114E+02 &  2.122E+00 & 0 &0 & 3.112E+03 &  2.659E+02 \\
25 & PDMP-N10**7 & isotropic-$\Delta$ & 500 & NA & 5.092E+02 &  2.132E+00 & 0 &0 & 2.328E+04 &  2.978E+03 \\
\hline
50 & PDMP-N10**5 & standard-$\Delta$ & 50 & NA & 5.391E+01 &  5.793E-01 & 0 &0 & 3.702E+00 &  7.443E-02 \\
50 & PDMP-N10**6 & standard-$\Delta$ & 50 & NA & 5.285E+01 &  4.425E-01 & 0 &0 & 2.907E+01 &  3.634E-01 \\
\hdashline
50 & PDMP-N10**5 & standard-$\Delta$ & 70 & NA & 7.457E+01 &  6.983E-01 & 0 &0 & 6.799E+00 &  1.791E-01 \\
50 & PDMP-N10**6 & standard-$\Delta$ & 70 & NA & 7.292E+01 &  4.885E-01 & 0 &0 & 5.099E+01 &  6.833E-01 \\
\hdashline
50 & PDMP-N10**5 & standard-$\Delta$ & 100 & NA & 1.061E+02 &  1.022E+00 & 0 &0 & 1.350E+01 &  2.935E-01 \\
50 & PDMP-N10**6 & standard-$\Delta$ & 100 & NA & 1.037E+02 &  6.735E-01 & 0 &0 & 9.465E+01 &  9.332E-01 \\
\hdashline
50 & PDMP-N10**5 & standard-$\Delta$ & 500 & NA & 5.179E+02 &  3.678E+00 & 0 &0 & 7.727E+02 &  6.141E+01 \\
50 & PDMP-N10**6 & standard-$\Delta$ & 500 & NA & 5.053E+02 &  2.175E+00 & 0 &0 & 3.175E+03 &  1.058E+02 \\
25 & PDMP-N10**7 & standard-$\Delta$ & 500 & NA & 5.050E+02 &  1.624E+00 & 0 &0 & 2.744E+04 &  3.650E+03 \\


==> fig-pdm-all-v2/batch-aggregated-volumes.tex <==
50 & PDMP-N10**5 & cube & 50 & NA &1.126e+15 & 1.048e+15 & 1.218e+15 & 1.114e+15 & 3.989e+13 &  2.731E-02 &  1.931E-02 \\
50 & PDMP-N10**6 & cube & 50 & NA &1.126e+15 & 1.052e+15 & 1.202e+15 & 1.134e+15 & 3.604e+13 &  2.248E-02 &  1.869E-02 \\
\hdashline
50 & PDMP-N10**5 & cube & 70 & NA &1.181e+21 & 1.018e+21 & 1.324e+21 & 1.168e+21 & 6.612e+19 &  3.442E-02 &  3.414E-02 \\
50 & PDMP-N10**6 & cube & 70 & NA &1.181e+21 & 1.122e+21 & 1.272e+21 & 1.187e+21 & 3.539e+19 &  2.198E-02 &  1.857E-02 \\
\hdashline
50 & PDMP-N10**5 & cube & 100 & NA &1.268e+30 & 1.08e+30 & 1.505e+30 & 1.253e+30 & 8.121e+28 &  4.421E-02 &  4.029E-02 \\
50 & PDMP-N10**6 & cube & 100 & NA &1.268e+30 & 1.189e+30 & 1.332e+30 & 1.259e+30 & 3.594e+28 &  2.104E-02 &  1.544E-02 \\
\hdashline
50 & PDMP-N10**5 & cube & 500 & NA &3.273e+150 & 1.193e+150 & 6.295e+150 & 2.656e+150 & 1.173e+150 &  2.955E-01 &  2.033E-01 \\
50 & PDMP-N10**6 & cube & 500 & NA &3.273e+150 & 2.289e+150 & 4.084e+150 & 3.197e+150 & 4.064e+149 &  9.948E-02 &  6.933E-02 \\
25 & PDMP-N10**7 & cube & 500 & NA &3.273e+150 & 2.868e+150 & 3.593e+150 & 3.25e+150 & 1.666e+149 &  3.969E-02 &  3.274E-02 \\
\hline
50 & PDMP-N10**5 & isotropic-$\Delta$ & 50 & NA &3.421e+21 & 2.994e+21 & 4.044e+21 & 3.415e+21 & 2.467e+20 &  4.751E-02 &  4.353E-02 \\
50 & PDMP-N10**6 & isotropic-$\Delta$ & 50 & NA &3.421e+21 & 3.213e+21 & 3.566e+21 & 3.396e+21 & 9.747e+19 &  2.394E-02 &  1.708E-02 \\
\hdashline
50 & PDMP-N10**5 & isotropic-$\Delta$ & 70 & NA &1.658e+30 & 1.424e+30 & 1.994e+30 & 1.645e+30 & 1.321e+29 &  5.922E-02 &  4.932E-02 \\
50 & PDMP-N10**6 & isotropic-$\Delta$ & 70 & NA &1.658e+30 & 1.489e+30 & 1.819e+30 & 1.657e+30 & 8.023e+28 &  3.827E-02 &  2.776E-02 \\
\hdashline
50 & PDMP-N10**5 & isotropic-$\Delta$ & 100 & NA &1.771e+43 & 1.31e+43 & 2.145e+43 & 1.697e+43 & 1.819e+42 &  6.347E-02 &  6.675E-02 \\
50 & PDMP-N10**6 & isotropic-$\Delta$ & 100 & NA &1.771e+43 & 1.586e+43 & 1.948e+43 & 1.754e+43 & 8.567e+41 &  3.324E-02 &  2.850E-02 \\
\hdashline
50 & PDMP-N10**5 & isotropic-$\Delta$ & 500 & NA &9.235e+216 & 1.311e+216 & 2.292e+217 & 5.133e+216 & 4.806e+216 &  5.364E-01 &  3.031E-01 \\
50 & PDMP-N10**6 & isotropic-$\Delta$ & 500 & NA &9.235e+216 & 4.967e+216 & 1.38e+217 & 9.04e+216 & 1.938e+216 &  1.410E-01 &  1.284E-01 \\
25 & PDMP-N10**7 & isotropic-$\Delta$ & 500 & NA &9.235e+216 & 7.16e+216 & 1.123e+217 & 9.113e+216 & 9.188e+215 &  4.407E-02 &  6.582E-02 \\
\hline
50 & PDMP-N10**5 & standard-$\Delta$ & 50 & NA &3.288e-65 & 2.87e-65 & 3.858e-65 & 3.195e-65 & 2.154e-66 &  4.624E-02 &  3.904E-02 \\
50 & PDMP-N10**6 & standard-$\Delta$ & 50 & NA &3.288e-65 & 3.031e-65 & 3.502e-65 & 3.315e-65 & 1.147e-66 &  2.760E-02 &  1.890E-02 \\
\hdashline
50 & PDMP-N10**5 & standard-$\Delta$ & 70 & NA &8.348e-101 & 6.38e-101 & 1.037e-100 & 8.317e-101 & 9.19e-102 &  9.248E-02 &  6.139E-02 \\
50 & PDMP-N10**6 & standard-$\Delta$ & 70 & NA &8.348e-101 & 7.74e-101 & 9.007e-101 & 8.356e-101 & 3.242e-102 &  2.575E-02 &  2.276E-02 \\
\hdashline
50 & PDMP-N10**5 & standard-$\Delta$ & 100 & NA &1.072e-158 & 7.873e-159 & 1.537e-158 & 1.081e-158 & 1.752e-159 &  1.054E-01 &  9.916E-02 \\
50 & PDMP-N10**6 & standard-$\Delta$ & 100 & NA &1.072e-158 & 9.567e-159 & 1.177e-158 & 1.085e-158 & 5.308e-160 &  2.856E-02 &  2.991E-02 \\
\hdashline
50 & PDMP-N10**5 & standard-$\Delta$ & 500 & NA &8.196e-1135 & 1.431e-1135 & 2.249e-1134 & 5.193e-1135 & 4.255e-1135 &  4.676E-01 &  3.004E-01 \\
50 & PDMP-N10**6 & standard-$\Delta$ & 500 & NA &8.196e-1135 & 4.838e-1135 & 1.546e-1134 & 7.885e-1135 & 1.859e-1135 &  1.504E-01 &  1.487E-01 \\
25 & PDMP-N10**7 & standard-$\Delta$ & 500 & NA &8.196e-1135 & 7.02e-1135 & 1.037e-1134 & 8.099e-1135 & 7.98e-1136 &  7.312E-02 &  6.213E-02 \\


==> fig-pdm-test-hd/batch-aggregated-misc.tex <==
5 & PDM-N10**5 & cube & 500 & NA & 9.999E+04 &  1.304E+00 &  NA & NA & NA & NA & NA & NA & 9.340E+02 &  9.251E+01 \\
5 & PDM-N10**6 & cube & 500 & NA & 1.000E+06 &  1.817E+00 &  NA & NA & NA & NA & NA & NA & 4.066E+03 &  1.124E+02 \\
\hline
4 & PDM-N10**5 & isotropic-$\Delta$ & 500 & NA & 9.998E+04 &  2.380E+00 &  NA & NA & NA & NA & NA & NA & 7.497E+02 &  5.269E+01 \\
5 & PDM-N10**6 & isotropic-$\Delta$ & 500 & NA & 1.000E+06 &  1.304E+00 &  NA & NA & NA & NA & NA & NA & 2.524E+03 &  1.374E+02 \\
\hline
5 & PDM-N10**5 & standard-$\Delta$ & 500 & NA & 9.998E+04 &  1.304E+00 &  NA & NA & NA & NA & NA & NA & 7.187E+02 &  3.684E+01 \\
5 & PDM-N10**6 & standard-$\Delta$ & 500 & NA & 1.000E+06 &  1.140E+00 &  NA & NA & NA & NA & NA & NA & 2.588E+03 &  1.506E+02 \\


==> fig-pdm-test-hd/batch-aggregated-volumes.tex <==
5 & PDM-N10**5 & cube & 500 & NA &3.273e+150 & 1.879e+150 & 2.69e+150 & 2.204e+150 & 2.977e+149 &  3.268E-01 &  9.094E-02 \\
5 & PDM-N10**6 & cube & 500 & NA &3.273e+150 & 2.77e+150 & 3.367e+150 & 3.196e+150 & 2.273e+149 &  2.855E-02 &  5.785E-02 \\
\hline
4 & PDM-N10**5 & isotropic-$\Delta$ & 500 & NA &9.235e+216 & 5.019e+216 & 8.998e+216 & 7.307e+216 & 1.662e+216 &  3.002E-01 &  1.800E-01 \\
5 & PDM-N10**6 & isotropic-$\Delta$ & 500 & NA &9.235e+216 & 7.703e+216 & 1.246e+217 & 8.144e+216 & 2.138e+216 &  1.623E-01 &  9.025E-02 \\
\hline
5 & PDM-N10**5 & standard-$\Delta$ & 500 & NA &8.196e-1135 & 3.665e-1135 & 4.682e-1135 & 3.756e-1135 & 4.166e-1136 &  5.417E-01 &  5.083E-02 \\
5 & PDM-N10**6 & standard-$\Delta$ & 500 & NA &8.196e-1135 & 5.665e-1135 & 8.706e-1135 & 5.886e-1135 & 1.265e-1135 &  2.818E-01 &  1.001E-01 \\


==> fig-pdm-test/batch-aggregated-misc.tex <==
5 & PDM-N10**4 & cube & 10 & NA &10000 & 1.378E+01 &  3.113E-01 & 0 &0 & 6.633E-02 &  1.606E-03 \\
\hdashline
5 & PDM-N10**4 & cube & 20 & NA &9999 & 2.443E+01 &  5.807E-01 & 0 &0 & 1.547E-01 &  5.184E-03 \\
\hline
5 & PDM-N10**4 & isotropic-$\Delta$ & 10 & NA &9999 & 1.387E+01 &  2.696E-01 & 0 &0 & 7.172E-02 &  5.735E-03 \\
\hdashline
5 & PDM-N10**4 & isotropic-$\Delta$ & 20 & NA &9998 & 2.664E+01 &  9.298E-01 & 0 &0 & 1.845E-01 &  1.306E-02 \\
\hline
5 & PDM-N10**4 & standard-$\Delta$ & 10 & NA &9999 & 1.373E+01 &  2.742E-01 & 0 &0 & 6.664E-02 &  4.986E-03 \\
\hdashline
5 & PDM-N10**4 & standard-$\Delta$ & 20 & NA &9997 & 2.566E+01 &  1.381E+00 & 0 &0 & 1.641E-01 &  1.717E-02 \\


==> fig-pdm-test/batch-aggregated-volumes.tex <==
5 & PDM-N10**4 & cube & 10 & NA &1024.0 & 998.3 & 1063.0 & 1004.0 & 28.47 &  1.926E-02 &  8.932E-03 \\
\hdashline
5 & PDM-N10**4 & cube & 20 & NA &1.049e+6 & 1.038e+6 & 1.104e+6 & 1.083e+6 & 2.536e+4 &  3.271E-02 &  1.764E-02 \\
\hline
5 & PDM-N10**4 & isotropic-$\Delta$ & 10 & NA &1.472e+4 & 1.356e+4 & 1.592e+4 & 1.444e+4 & 1066.0 &  6.771E-02 &  2.529E-02 \\
\hdashline
5 & PDM-N10**4 & isotropic-$\Delta$ & 20 & NA &3.217e+8 & 3.008e+8 & 3.391e+8 & 3.084e+8 & 1.568e+7 &  5.393E-02 &  1.645E-02 \\
\hline
5 & PDM-N10**4 & standard-$\Delta$ & 10 & NA &2.756e-7 & 2.695e-7 & 3.0e-7 & 2.823e-7 & 1.253e-8 &  2.456E-02 &  3.465E-02 \\
\hdashline
5 & PDM-N10**4 & standard-$\Delta$ & 20 & NA &4.11e-19 & 3.662e-19 & 4.814e-19 & 4.089e-19 & 4.628e-20 &  9.936E-02 &  7.302E-02 \\


==> merged/batch-UNK-misc.tex <==
5 & PDM-N10**2 & cube & 10 & NA & 1.000E+02 &  4.472E-01 &  NA & NA & NA & NA & NA & NA & 1.640E+00 &  2.067E-01 \\
\hdashline
5 & PDM-N10**2 & cube & 20 & NA & 9.900E+01 &  0.000E+00 &  NA & NA & NA & NA & NA & NA & 7.555E+00 &  1.533E+00 \\


==> merged/batch-UNK-volumes.tex <==
5 & PDM-N10**2 & cube & 10 & NA &1.024E+03 &  7.371E+02 &  9.703E+02 &  8.830E+02 &  8.816E+01 &  1.377E-01 &  8.609E-02 \\
\hdashline
5 & PDM-N10**2 & cube & 20 & NA &1.049E+06 &  4.079E+05 &  1.554E+06 &  9.223E+05 &  4.458E+05 &  2.707E-01 &  2.009E-01 \\


==> merged/batch-aggregated-misc.tex <==
10 & PDM-N10**5 & cube & 50 & NA & 1.000E+05 &  9.661E-01 &  NA & NA & NA & NA & NA & NA & 1.441E+01 &  2.246E+00 \\
10 & PDM-N10**6 & cube & 50 & NA & 1.000E+06 &  7.379E-01 &  NA & NA & NA & NA & NA & NA & 1.110E+02 &  1.544E+01 \\
10 & PDM-N10**7 & cube & 50 & NA & 1.000E+07 &  5.164E-01 &  NA & NA & NA & NA & NA & NA & 1.107E+03 &  1.330E+02 \\
\hdashline
10 & PDM-N10**5 & cube & 70 & NA & 1.000E+05 &  7.888E-01 &  NA & NA & NA & NA & NA & NA & 3.314E+01 &  2.522E+00 \\
10 & PDM-N10**6 & cube & 70 & NA & 1.000E+06 &  6.325E-01 &  NA & NA & NA & NA & NA & NA & 2.411E+02 &  2.527E+01 \\
10 & PDM-N10**7 & cube & 70 & NA & 1.000E+07 &  6.992E-01 &  NA & NA & NA & NA & NA & NA & 2.282E+03 &  3.013E+02 \\
\hdashline
10 & PDM-N10**5 & cube & 100 & NA & 1.000E+05 &  7.071E-01 &  NA & NA & NA & NA & NA & NA & 9.261E+01 &  8.977E+00 \\
10 & PDM-N10**6 & cube & 100 & NA & 1.000E+06 &  8.233E-01 &  NA & NA & NA & NA & NA & NA & 6.781E+02 &  6.337E+01 \\
10 & PDM-N10**7 & cube & 100 & NA & 1.000E+07 &  8.756E-01 &  NA & NA & NA & NA & NA & NA & 6.682E+03 &  6.830E+02 \\
\hline
10 & PDM-N10**5 & isotropic-$\Delta$ & 50 & NA & 1.000E+05 &  7.379E-01 &  NA & NA & NA & NA & NA & NA & 9.262E+00 &  8.458E-01 \\
10 & PDM-N10**6 & isotropic-$\Delta$ & 50 & NA & 1.000E+06 &  8.233E-01 &  NA & NA & NA & NA & NA & NA & 5.573E+01 &  1.096E+01 \\
10 & PDM-N10**7 & isotropic-$\Delta$ & 50 & NA & 1.000E+07 &  7.379E-01 &  NA & NA & NA & NA & NA & NA & 6.901E+02 &  9.153E+01 \\
\hdashline
10 & PDM-N10**5 & isotropic-$\Delta$ & 70 & NA & 1.000E+05 &  8.756E-01 &  NA & NA & NA & NA & NA & NA & 1.716E+01 &  3.571E+00 \\
10 & PDM-N10**6 & isotropic-$\Delta$ & 70 & NA & 1.000E+06 &  7.888E-01 &  NA & NA & NA & NA & NA & NA & 9.776E+01 &  2.341E+01 \\
10 & PDM-N10**7 & isotropic-$\Delta$ & 70 & NA & 1.000E+07 &  1.059E+00 &  NA & NA & NA & NA & NA & NA & 1.213E+03 &  3.046E+02 \\
\hdashline
10 & PDM-N10**5 & isotropic-$\Delta$ & 100 & NA & 1.000E+05 &  7.888E-01 &  NA & NA & NA & NA & NA & NA & 2.668E+01 &  7.804E-01 \\
10 & PDM-N10**6 & isotropic-$\Delta$ & 100 & NA & 1.000E+06 &  8.756E-01 &  NA & NA & NA & NA & NA & NA & 1.254E+02 &  2.296E+00 \\
10 & PDM-N10**7 & isotropic-$\Delta$ & 100 & NA & 1.000E+07 &  9.661E-01 &  NA & NA & NA & NA & NA & NA & 1.157E+03 &  2.915E+01 \\
\hline
10 & PDM-N10**5 & standard-$\Delta$ & 50 & NA & 1.000E+05 &  6.749E-01 &  NA & NA & NA & NA & NA & NA & 1.041E+01 &  7.839E-01 \\
10 & PDM-N10**6 & standard-$\Delta$ & 50 & NA & 1.000E+06 &  6.325E-01 &  NA & NA & NA & NA & NA & NA & 7.706E+01 &  8.331E+00 \\
10 & PDM-N10**7 & standard-$\Delta$ & 50 & NA & 1.000E+07 &  8.498E-01 &  NA & NA & NA & NA & NA & NA & 6.948E+02 &  5.901E+01 \\
\hdashline
10 & PDM-N10**5 & standard-$\Delta$ & 70 & NA & 1.000E+05 &  1.197E+00 &  NA & NA & NA & NA & NA & NA & 2.501E+01 &  2.495E+00 \\
10 & PDM-N10**6 & standard-$\Delta$ & 70 & NA & 1.000E+06 &  1.370E+00 &  NA & NA & NA & NA & NA & NA & 1.803E+02 &  2.269E+01 \\
10 & PDM-N10**7 & standard-$\Delta$ & 70 & NA & 1.000E+07 &  9.718E-01 &  NA & NA & NA & NA & NA & NA & 1.806E+03 &  1.945E+02 \\
\hdashline
10 & PDM-N10**5 & standard-$\Delta$ & 100 & NA & 1.000E+05 &  8.165E-01 &  NA & NA & NA & NA & NA & NA & 4.618E+01 &  4.413E+00 \\
10 & PDM-N10**6 & standard-$\Delta$ & 100 & NA & 1.000E+06 &  7.888E-01 &  NA & NA & NA & NA & NA & NA & 2.988E+02 &  4.801E+01 \\
10 & PDM-N10**7 & standard-$\Delta$ & 100 & NA & 1.000E+07 &  6.992E-01 &  NA & NA & NA & NA & NA & NA & 3.258E+03 &  4.976E+02 \\


==> merged/batch-aggregated-volumes.tex <==
10 & PDM-N10**5 & cube & 50 & NA &1.126E+15 &  1.049E+15 &  1.162E+15 &  1.116E+15 &  3.573E+13 &  2.567E-02 &  2.048E-02 \\
10 & PDM-N10**6 & cube & 50 & NA &1.126E+15 &  1.089E+15 &  1.153E+15 &  1.128E+15 &  1.761E+13 &  8.500E-03 &  1.034E-02 \\
10 & PDM-N10**7 & cube & 50 & NA &1.126E+15 &  1.090E+15 &  1.180E+15 &  1.149E+15 &  3.261E+13 &  3.086E-02 &  9.607E-03 \\
\hdashline
10 & PDM-N10**5 & cube & 70 & NA &1.181E+21 &  1.099E+21 &  1.266E+21 &  1.198E+21 &  5.644E+19 &  5.072E-02 &  2.454E-02 \\
10 & PDM-N10**6 & cube & 70 & NA &1.181E+21 &  1.107E+21 &  1.231E+21 &  1.165E+21 &  3.776E+19 &  2.514E-02 &  1.918E-02 \\
10 & PDM-N10**7 & cube & 70 & NA &1.181E+21 &  1.119E+21 &  1.218E+21 &  1.181E+21 &  3.156E+19 &  2.404E-02 &  1.804E-02 \\
\hdashline
10 & PDM-N10**5 & cube & 100 & NA &1.268E+30 &  1.172E+30 &  1.407E+30 &  1.248E+30 &  7.748E+28 &  6.082E-02 &  3.318E-02 \\
10 & PDM-N10**6 & cube & 100 & NA &1.268E+30 &  1.209E+30 &  1.321E+30 &  1.298E+30 &  3.479E+28 &  3.243E-02 &  1.652E-02 \\
10 & PDM-N10**7 & cube & 100 & NA &1.268E+30 &  1.231E+30 &  1.343E+30 &  1.256E+30 &  3.571E+28 &  1.613E-02 &  1.643E-02 \\
\hline
10 & PDM-N10**5 & isotropic-$\Delta$ & 50 & NA &3.421E+21 &  2.961E+21 &  3.846E+21 &  3.362E+21 &  3.226E+20 &  7.915E-02 &  4.415E-02 \\
10 & PDM-N10**6 & isotropic-$\Delta$ & 50 & NA &3.421E+21 &  2.550E+21 &  3.490E+21 &  3.332E+21 &  3.404E+20 &  3.723E-02 &  9.223E-02 \\
10 & PDM-N10**7 & isotropic-$\Delta$ & 50 & NA &3.421E+21 &  3.354E+21 &  3.558E+21 &  3.438E+21 &  6.626E+19 &  6.716E-03 &  1.437E-02 \\
\hdashline
10 & PDM-N10**5 & isotropic-$\Delta$ & 70 & NA &1.658E+30 &  5.773E+29 &  1.557E+30 &  1.404E+30 &  3.292E+29 &  2.945E-01 &  1.985E-01 \\
10 & PDM-N10**6 & isotropic-$\Delta$ & 70 & NA &1.658E+30 &  6.948E+29 &  1.884E+30 &  1.202E+30 &  3.674E+29 &  3.992E-01 &  1.649E-01 \\
10 & PDM-N10**7 & isotropic-$\Delta$ & 70 & NA &1.658E+30 &  1.182E+30 &  1.841E+30 &  1.567E+30 &  1.720E+29 &  7.554E-02 &  7.769E-02 \\
\hdashline
10 & PDM-N10**5 & isotropic-$\Delta$ & 100 & NA &1.771E+43 &  5.653E+40 &  1.521E+42 &  3.327E+41 &  4.900E+41 &  9.835E-01 &  2.767E-02 \\
10 & PDM-N10**6 & isotropic-$\Delta$ & 100 & NA &1.771E+43 &  1.009E+42 &  6.611E+43 &  1.773E+42 &  2.022E+43 &  9.314E-01 &  6.086E-01 \\
10 & PDM-N10**7 & isotropic-$\Delta$ & 100 & NA &1.771E+43 &  2.245E+41 &  3.930E+43 &  1.770E+42 &  1.198E+43 &  9.514E-01 &  1.507E-01 \\
\hline
10 & PDM-N10**5 & standard-$\Delta$ & 50 & NA &3.288E-65 &  1.633E-65 &  8.708E-65 &  4.299E-65 &  2.446E-65 &  4.654E-01 &  5.181E-01 \\
10 & PDM-N10**6 & standard-$\Delta$ & 50 & NA &3.288E-65 &  2.093E-65 &  3.856E-65 &  3.089E-65 &  5.391E-66 &  1.045E-01 &  9.433E-02 \\
10 & PDM-N10**7 & standard-$\Delta$ & 50 & NA &3.288E-65 &  2.700E-65 &  3.512E-65 &  2.949E-65 &  2.679E-66 &  1.110E-01 &  4.937E-02 \\
\hdashline
10 & PDM-N10**5 & standard-$\Delta$ & 70 & NA &8.348E-101 &  1.042E-101 &  6.608E-101 &  3.235E-101 &  1.774E-101 &  8.064E-01 &  2.126E-01 \\
10 & PDM-N10**6 & standard-$\Delta$ & 70 & NA &8.348E-101 &  1.608E-101 &  1.381E-100 &  5.294E-101 &  3.531E-101 &  4.475E-01 &  2.512E-01 \\
10 & PDM-N10**7 & standard-$\Delta$ & 70 & NA &8.348E-101 &  2.828E-101 &  1.072E-99 &  5.518E-101 &  3.247E-100 &  5.797E-01 &  3.603E+00 \\
\hdashline
10 & PDM-N10**5 & standard-$\Delta$ & 100 & NA &1.072E-158 &  5.039E-162 &  5.692E-160 &  3.614E-161 &  2.123E-160 &  9.981E-01 &  1.981E-02 \\
10 & PDM-N10**6 & standard-$\Delta$ & 100 & NA &1.072E-158 &  1.388E-161 &  4.289E-159 &  1.296E-160 &  1.325E-159 &  9.912E-01 &  1.237E-01 \\
10 & PDM-N10**7 & standard-$\Delta$ & 100 & NA &1.072E-158 &  1.615E-160 &  1.720E-159 &  5.407E-160 &  5.328E-160 &  9.651E-01 &  4.972E-02 \\


==> pdm-ais-prod0/batch-aggregated-misc-d500.tex <==
48 & PDMP-N10**5 & cube & 100 & NA & 1.084E+02 &  3.456E+00 & 0 &0 & 1.506E+01 &  4.787E-01 \\
48 & PDMP-N10**6 & cube & 100 & NA & 1.094E+02 &  3.739E+00 & 0 &0 & 1.261E+02 &  3.464E+00 \\
\hdashline
48 & PDMP-N10**5 & cube & 500 & NA & 5.187E+02 &  5.499E+00 & 0 &0 & 1.127E+03 &  6.796E+01 \\
48 & PDMP-N10**6 & cube & 500 & NA & 5.155E+02 &  4.751E+00 & 0 &0 & 6.595E+03 &  6.420E+02 \\
24 & PDMP-N10**7 & cube & 500 & NA & 5.123E+02 &  5.283E+00 & 0 &0 & 5.729E+04 &  1.107E+04 \\
\hline
48 & PDMP-N10**5 & isotropic-$\Delta$ & 100 & NA & 1.070E+02 &  1.309E+00 & 0 &0 & 1.368E+01 &  3.791E-01 \\
48 & PDMP-N10**6 & isotropic-$\Delta$ & 100 & NA & 1.047E+02 &  1.054E+00 & 0 &0 & 9.637E+01 &  1.424E+00 \\
\hdashline
48 & PDMP-N10**5 & isotropic-$\Delta$ & 500 & NA & 5.240E+02 &  3.540E+00 & 0 &0 & 7.503E+02 &  4.174E+01 \\
48 & PDMP-N10**6 & isotropic-$\Delta$ & 500 & NA & 5.114E+02 &  2.122E+00 & 0 &0 & 3.112E+03 &  2.659E+02 \\
24 & PDMP-N10**7 & isotropic-$\Delta$ & 500 & NA & 5.092E+02 &  2.132E+00 & 0 &0 & 2.328E+04 &  2.978E+03 \\
\hline
48 & PDMP-N10**5 & standard-$\Delta$ & 100 & NA & 1.061E+02 &  1.022E+00 & 0 &0 & 1.350E+01 &  2.935E-01 \\
48 & PDMP-N10**6 & standard-$\Delta$ & 100 & NA & 1.037E+02 &  6.735E-01 & 0 &0 & 9.465E+01 &  9.332E-01 \\
\hdashline
48 & PDMP-N10**5 & standard-$\Delta$ & 500 & NA & 5.179E+02 &  3.678E+00 & 0 &0 & 7.727E+02 &  6.141E+01 \\
48 & PDMP-N10**6 & standard-$\Delta$ & 500 & NA & 5.053E+02 &  2.175E+00 & 0 &0 & 3.175E+03 &  1.058E+02 \\
24 & PDMP-N10**7 & standard-$\Delta$ & 500 & NA & 5.050E+02 &  1.624E+00 & 0 &0 & 2.744E+04 &  3.650E+03 \\


==> pdm-ais-prod0/batch-aggregated-misc.tex <==
24 & PDMP-N9.4e+04 & cube & 50 & NA & 5.495E+01 &  7.835E-01 & 0 &0 & 3.785E+00 &  5.925E-02 \\
\hdashline
24 & PDMP-N1.6e+05 & cube & 70 & NA & 7.559E+01 &  1.491E+00 & 0 &0 & 1.165E+01 &  2.350E-01 \\
\hdashline
24 & PDMP-N1.6e+05 & cube & 100 & NA & 1.074E+02 &  2.305E+00 & 0 &0 & 2.200E+01 &  3.762E-01 \\
\hdashline
24 & PDMP-N2.8e+05 & cube & 140 & NA & 1.513E+02 &  4.228E+00 & 0 &0 & 7.324E+01 &  1.451E+00 \\
\hdashline
24 & PDMP-N5.6e+05 & cube & 175 & NA & 1.940E+02 &  5.043E+00 & 0 &0 & 2.214E+02 &  3.170E+00 \\
\hdashline
24 & PDMP-N2.2e+06 & cube & 250 & NA & 2.670E+02 &  4.294E+00 & 0 &0 & 1.733E+03 &  2.984E+01 \\
\hline
24 & PDMP-N4.0e+05 & isotropic-$\Delta$ & 50 & NA & 5.358E+01 &  4.274E-01 & 0 &0 & 1.181E+01 &  1.189E-01 \\
\hdashline
24 & PDMP-N6.0e+05 & isotropic-$\Delta$ & 70 & NA & 7.376E+01 &  7.949E-01 & 0 &0 & 3.111E+01 &  3.072E-01 \\
\hdashline
24 & PDMP-N1.2e+06 & isotropic-$\Delta$ & 100 & NA & 1.046E+02 &  8.205E-01 & 0 &0 & 1.127E+02 &  1.351E+00 \\
\hdashline
24 & PDMP-N2.2e+06 & isotropic-$\Delta$ & 140 & NA & 1.470E+02 &  2.593E+00 & 0 &0 & 4.120E+02 &  4.911E+00 \\
\hdashline
24 & PDMP-N3.3e+06 & isotropic-$\Delta$ & 175 & NA & 1.848E+02 &  2.308E+00 & 0 &0 & 8.700E+02 &  6.177E+00 \\
\hdashline
24 & PDMP-N5.6e+06 & isotropic-$\Delta$ & 250 & NA & 2.611E+02 &  2.033E+00 & 0 &0 & 3.000E+03 &  3.289E+01 \\
\hline
24 & PDMP-N6.0e+05 & standard-$\Delta$ & 50 & NA & 5.294E+01 &  3.976E-01 & 0 &0 & 1.695E+01 &  2.969E-01 \\
\hdashline
24 & PDMP-N8.9e+05 & standard-$\Delta$ & 70 & NA & 7.316E+01 &  4.611E-01 & 0 &0 & 4.469E+01 &  4.739E-01 \\
\hdashline
24 & PDMP-N9.9e+05 & standard-$\Delta$ & 100 & NA & 1.034E+02 &  1.000E+00 & 0 &0 & 9.205E+01 &  9.745E-01 \\
\hdashline
24 & PDMP-N2.2e+06 & standard-$\Delta$ & 140 & NA & 1.441E+02 &  1.072E+00 & 0 &0 & 3.975E+02 &  2.793E+00 \\
\hdashline
24 & PDMP-N3.3e+06 & standard-$\Delta$ & 175 & NA & 1.796E+02 &  1.610E+00 & 0 &0 & 8.413E+02 &  7.220E+00 \\
\hdashline
24 & PDMP-N4.7e+06 & standard-$\Delta$ & 250 & NA & 2.569E+02 &  1.657E+00 & 0 &0 & 2.446E+03 &  2.550E+01 \\


==> pdm-ais-prod0/batch-aggregated-volumes-d500.tex <==
48 & PDMP-N10**5 & cube & 100 & NA &1.268e+30 & 1.08e+30 & 1.505e+30 & 1.253e+30 & 8.121e+28 &  4.421E-02 &  4.029E-02 \\
48 & PDMP-N10**6 & cube & 100 & NA &1.268e+30 & 1.189e+30 & 1.332e+30 & 1.259e+30 & 3.594e+28 &  2.104E-02 &  1.544E-02 \\
\hdashline
48 & PDMP-N10**5 & cube & 500 & NA &3.273e+150 & 1.193e+150 & 6.295e+150 & 2.656e+150 & 1.173e+150 &  2.955E-01 &  2.033E-01 \\
48 & PDMP-N10**6 & cube & 500 & NA &3.273e+150 & 2.289e+150 & 4.084e+150 & 3.197e+150 & 4.064e+149 &  9.948E-02 &  6.933E-02 \\
24 & PDMP-N10**7 & cube & 500 & NA &3.273e+150 & 2.868e+150 & 3.593e+150 & 3.25e+150 & 1.666e+149 &  3.969E-02 &  3.274E-02 \\
\hline
48 & PDMP-N10**5 & isotropic-$\Delta$ & 100 & NA &1.771e+43 & 1.31e+43 & 2.145e+43 & 1.697e+43 & 1.819e+42 &  6.347E-02 &  6.675E-02 \\
48 & PDMP-N10**6 & isotropic-$\Delta$ & 100 & NA &1.771e+43 & 1.586e+43 & 1.948e+43 & 1.754e+43 & 8.567e+41 &  3.324E-02 &  2.850E-02 \\
\hdashline
48 & PDMP-N10**5 & isotropic-$\Delta$ & 500 & NA &9.235e+216 & 1.311e+216 & 2.292e+217 & 5.133e+216 & 4.806e+216 &  5.364E-01 &  3.031E-01 \\
48 & PDMP-N10**6 & isotropic-$\Delta$ & 500 & NA &9.235e+216 & 4.967e+216 & 1.38e+217 & 9.04e+216 & 1.938e+216 &  1.410E-01 &  1.284E-01 \\
24 & PDMP-N10**7 & isotropic-$\Delta$ & 500 & NA &9.235e+216 & 7.16e+216 & 1.123e+217 & 9.113e+216 & 9.188e+215 &  4.407E-02 &  6.582E-02 \\
\hline
48 & PDMP-N10**5 & standard-$\Delta$ & 100 & NA &1.072e-158 & 7.873e-159 & 1.537e-158 & 1.081e-158 & 1.752e-159 &  1.054E-01 &  9.916E-02 \\
48 & PDMP-N10**6 & standard-$\Delta$ & 100 & NA &1.072e-158 & 9.567e-159 & 1.177e-158 & 1.085e-158 & 5.308e-160 &  2.856E-02 &  2.991E-02 \\
\hdashline
48 & PDMP-N10**5 & standard-$\Delta$ & 500 & NA &8.196e-1135 & 1.431e-1135 & 2.249e-1134 & 5.193e-1135 & 4.255e-1135 &  4.676E-01 &  3.004E-01 \\
48 & PDMP-N10**6 & standard-$\Delta$ & 500 & NA &8.196e-1135 & 4.838e-1135 & 1.546e-1134 & 7.885e-1135 & 1.859e-1135 &  1.504E-01 &  1.487E-01 \\
24 & PDMP-N10**7 & standard-$\Delta$ & 500 & NA &8.196e-1135 & 7.02e-1135 & 1.037e-1134 & 8.099e-1135 & 7.98e-1136 &  7.312E-02 &  6.213E-02 \\


==> pdm-ais-prod0/batch-aggregated-volumes.tex <==
24 & PDMP-N9.4e+04 & cube & 50 & NA &1.126e+15 & 1.078e+15 & 1.201e+15 & 1.141e+15 & 3.577e+13 &  2.776E-02 &  1.821E-02 \\
\hdashline
24 & PDMP-N1.6e+05 & cube & 70 & NA &1.181e+21 & 1.116e+21 & 1.285e+21 & 1.17e+21 & 4.758e+19 &  3.409E-02 &  2.180E-02 \\
\hdashline
24 & PDMP-N1.6e+05 & cube & 100 & NA &1.268e+30 & 1.163e+30 & 1.402e+30 & 1.301e+30 & 7.536e+28 &  5.391E-02 &  2.635E-02 \\
\hdashline
24 & PDMP-N2.8e+05 & cube & 140 & NA &1.394e+42 & 1.223e+42 & 1.515e+42 & 1.421e+42 & 8.874e+40 &  5.789E-02 &  2.908E-02 \\
\hdashline
24 & PDMP-N5.6e+05 & cube & 175 & NA &4.789e+52 & 4.355e+52 & 5.203e+52 & 4.8e+52 & 2.444e+51 &  3.792E-02 &  2.639E-02 \\
\hdashline
24 & PDMP-N2.2e+06 & cube & 250 & NA &1.809e+75 & 1.61e+75 & 2.001e+75 & 1.788e+75 & 1.002e+74 &  3.803E-02 &  2.940E-02 \\
\hline
24 & PDMP-N4.0e+05 & isotropic-$\Delta$ & 50 & NA &3.421e+21 & 3.141e+21 & 3.774e+21 & 3.396e+21 & 1.548e+20 &  1.730E-02 &  3.188E-02 \\
\hdashline
24 & PDMP-N6.0e+05 & isotropic-$\Delta$ & 70 & NA &1.658e+30 & 1.53e+30 & 2.159e+30 & 1.665e+30 & 1.213e+29 &  3.196E-02 &  5.981E-02 \\
\hdashline
24 & PDMP-N1.2e+06 & isotropic-$\Delta$ & 100 & NA &1.771e+43 & 1.638e+43 & 1.921e+43 & 1.785e+43 & 8.217e+41 &  3.135E-02 &  2.604E-02 \\
\hdashline
24 & PDMP-N2.2e+06 & isotropic-$\Delta$ & 140 & NA &4.167e+60 & 3.828e+60 & 4.594e+60 & 4.192e+60 & 2.086e+59 &  3.255E-02 &  3.099E-02 \\
\hdashline
24 & PDMP-N3.3e+06 & isotropic-$\Delta$ & 175 & NA &6.607e+75 & 6.021e+75 & 7.2e+75 & 6.454e+75 & 3.168e+74 &  4.124E-02 &  2.484E-02 \\
\hdashline
24 & PDMP-N5.6e+06 & isotropic-$\Delta$ & 250 & NA &2.466e+108 & 2.236e+108 & 2.777e+108 & 2.395e+108 & 1.195e+107 &  4.568E-02 &  3.035E-02 \\
\hline
24 & PDMP-N6.0e+05 & standard-$\Delta$ & 50 & NA &3.288e-65 & 3.051e-65 & 3.524e-65 & 3.326e-65 & 1.295e-66 &  2.400E-02 &  2.305E-02 \\
\hdashline
24 & PDMP-N8.9e+05 & standard-$\Delta$ & 70 & NA &8.348e-101 & 7.744e-101 & 8.874e-101 & 8.317e-101 & 3.161e-102 &  2.845E-02 &  2.119E-02 \\
\hdashline
24 & PDMP-N9.9e+05 & standard-$\Delta$ & 100 & NA &1.072e-158 & 9.717e-159 & 1.168e-158 & 1.043e-158 & 4.754e-160 &  3.823E-02 &  2.564E-02 \\
\hdashline
24 & PDMP-N2.2e+06 & standard-$\Delta$ & 140 & NA &7.428e-242 & 6.844e-242 & 7.971e-242 & 7.372e-242 & 3.246e-243 &  3.409E-02 &  2.358E-02 \\
\hdashline
24 & PDMP-N3.3e+06 & standard-$\Delta$ & 175 & NA &8.893e-319 & 8.237e-319 & 9.821e-319 & 8.808e-319 & 4.221e-320 &  2.818E-02 &  3.024E-02 \\
\hdashline
24 & PDMP-N4.7e+06 & standard-$\Delta$ & 250 & NA &3.093e-493 & 2.847e-493 & 3.41e-493 & 3.043e-493 & 1.613e-494 &  4.683E-02 &  3.086E-02 \\


==> pdm-ais-prod1/batch-aggregated-misc.tex <==
24 & PDMP-N9.7e+04 & cube & 50 & NA & 5.493E+01 &  1.022E+00 & 0 &0 & 3.911E+00 &  6.058E-02 \\
\hdashline
24 & PDMP-N1.6e+05 & cube & 70 & NA & 7.572E+01 &  1.704E+00 & 0 &0 & 1.203E+01 &  2.245E-01 \\
\hdashline
24 & PDMP-N1.7e+05 & cube & 100 & NA & 1.092E+02 &  3.831E+00 & 0 &0 & 2.458E+01 &  5.336E-01 \\
\hdashline
24 & PDMP-N5.8e+05 & cube & 140 & NA & 1.533E+02 &  4.603E+00 & 0 &0 & 1.437E+02 &  2.556E+00 \\
\hdashline
24 & PDMP-N5.2e+05 & cube & 175 & NA & 1.939E+02 &  5.588E+00 & 0 &0 & 2.069E+02 &  3.570E+00 \\
\hdashline
24 & PDMP-N2.2e+06 & cube & 250 & NA & 2.647E+02 &  4.139E+00 & 0 &0 & 1.701E+03 &  2.739E+01 \\
\hline
24 & PDMP-N3.9e+05 & isotropic-$\Delta$ & 50 & NA & 5.325E+01 &  5.144E-01 & 0 &0 & 1.148E+01 &  1.208E-01 \\
\hdashline
24 & PDMP-N5.8e+05 & isotropic-$\Delta$ & 70 & NA & 7.445E+01 &  7.062E-01 & 0 &0 & 3.049E+01 &  2.736E-01 \\
\hdashline
24 & PDMP-N1.2e+06 & isotropic-$\Delta$ & 100 & NA & 1.050E+02 &  1.317E+00 & 0 &0 & 1.101E+02 &  1.475E+00 \\
\hdashline
24 & PDMP-N2.3e+06 & isotropic-$\Delta$ & 140 & NA & 1.469E+02 &  1.928E+00 & 0 &0 & 4.285E+02 &  5.406E+00 \\
\hdashline
24 & PDMP-N3.4e+06 & isotropic-$\Delta$ & 175 & NA & 1.835E+02 &  2.296E+00 & 0 &0 & 9.006E+02 &  1.900E+01 \\
\hdashline
24 & PDMP-N5.4e+06 & isotropic-$\Delta$ & 250 & NA & 2.603E+02 &  2.409E+00 & 0 &0 & 2.895E+03 &  3.265E+01 \\
\hline
24 & PDMP-N5.8e+05 & standard-$\Delta$ & 50 & NA & 5.294E+01 &  5.319E-01 & 0 &0 & 1.656E+01 &  1.780E-01 \\
\hdashline
24 & PDMP-N8.7e+05 & standard-$\Delta$ & 70 & NA & 7.297E+01 &  6.392E-01 & 0 &0 & 4.372E+01 &  3.888E-01 \\
\hdashline
24 & PDMP-N9.7e+05 & standard-$\Delta$ & 100 & NA & 1.032E+02 &  9.591E-01 & 0 &0 & 9.010E+01 &  9.205E-01 \\
\hdashline
24 & PDMP-N2.3e+06 & standard-$\Delta$ & 140 & NA & 1.446E+02 &  1.217E+00 & 0 &0 & 4.111E+02 &  2.813E+00 \\
\hdashline
24 & PDMP-N3.4e+06 & standard-$\Delta$ & 175 & NA & 1.795E+02 &  1.346E+00 & 0 &0 & 8.715E+02 &  1.101E+01 \\
\hdashline
24 & PDMP-N4.8e+06 & standard-$\Delta$ & 250 & NA & 2.564E+02 &  1.509E+00 & 0 &0 & 2.520E+03 &  2.617E+01 \\


==> pdm-ais-prod1/batch-aggregated-volumes.tex <==
24 & PDMP-N9.7e+04 & cube & 50 & NA &1.126e+15 & 1.046e+15 & 1.222e+15 & 1.143e+15 & 4.438e+13 &  3.721E-02 &  2.200E-02 \\
\hdashline
24 & PDMP-N1.6e+05 & cube & 70 & NA &1.181e+21 & 1.082e+21 & 1.278e+21 & 1.178e+21 & 4.95e+19 &  2.536E-02 &  2.675E-02 \\
\hdashline
24 & PDMP-N1.7e+05 & cube & 100 & NA &1.268e+30 & 1.157e+30 & 1.367e+30 & 1.263e+30 & 5.088e+28 &  3.478E-02 &  2.647E-02 \\
\hdashline
24 & PDMP-N5.8e+05 & cube & 140 & NA &1.394e+42 & 1.304e+42 & 1.555e+42 & 1.38e+42 & 6.412e+40 &  4.208E-02 &  2.658E-02 \\
\hdashline
24 & PDMP-N5.2e+05 & cube & 175 & NA &4.789e+52 & 4.319e+52 & 5.192e+52 & 4.682e+52 & 2.261e+51 &  4.711E-02 &  2.681E-02 \\
\hdashline
24 & PDMP-N2.2e+06 & cube & 250 & NA &1.809e+75 & 1.661e+75 & 1.932e+75 & 1.805e+75 & 7.473e+73 &  3.396E-02 &  2.474E-02 \\
\hline
24 & PDMP-N3.9e+05 & isotropic-$\Delta$ & 50 & NA &3.421e+21 & 3.055e+21 & 3.732e+21 & 3.428e+21 & 1.692e+20 &  3.563E-02 &  3.061E-02 \\
\hdashline
24 & PDMP-N5.8e+05 & isotropic-$\Delta$ & 70 & NA &1.658e+30 & 1.547e+30 & 1.841e+30 & 1.647e+30 & 7.477e+28 &  4.118E-02 &  2.617E-02 \\
\hdashline
24 & PDMP-N1.2e+06 & isotropic-$\Delta$ & 100 & NA &1.771e+43 & 1.546e+43 & 1.865e+43 & 1.79e+43 & 8.501e+41 &  3.179E-02 &  2.851E-02 \\
\hdashline
24 & PDMP-N2.3e+06 & isotropic-$\Delta$ & 140 & NA &4.167e+60 & 3.59e+60 & 4.558e+60 & 4.096e+60 & 2.458e+59 &  4.215E-02 &  3.261E-02 \\
\hdashline
24 & PDMP-N3.4e+06 & isotropic-$\Delta$ & 175 & NA &6.607e+75 & 5.757e+75 & 7.069e+75 & 6.421e+75 & 3.292e+74 &  3.905E-02 &  2.930E-02 \\
\hdashline
24 & PDMP-N5.4e+06 & isotropic-$\Delta$ & 250 & NA &2.466e+108 & 2.331e+108 & 2.691e+108 & 2.482e+108 & 1.096e+107 &  4.183E-02 &  2.378E-02 \\
\hline
24 & PDMP-N5.8e+05 & standard-$\Delta$ & 50 & NA &3.288e-65 & 3.07e-65 & 3.602e-65 & 3.305e-65 & 1.447e-66 &  3.086E-02 &  2.554E-02 \\
\hdashline
24 & PDMP-N8.7e+05 & standard-$\Delta$ & 70 & NA &8.348e-101 & 7.647e-101 & 9.136e-101 & 8.321e-101 & 3.506e-102 &  1.486E-02 &  3.013E-02 \\
\hdashline
24 & PDMP-N9.7e+05 & standard-$\Delta$ & 100 & NA &1.072e-158 & 9.698e-159 & 1.179e-158 & 1.075e-158 & 5.651e-160 &  3.649E-02 &  3.058E-02 \\
\hdashline
24 & PDMP-N2.3e+06 & standard-$\Delta$ & 140 & NA &7.428e-242 & 6.623e-242 & 8.31e-242 & 7.349e-242 & 3.798e-243 &  3.372E-02 &  3.315E-02 \\
\hdashline
24 & PDMP-N3.4e+06 & standard-$\Delta$ & 175 & NA &8.893e-319 & 7.979e-319 & 9.688e-319 & 8.922e-319 & 4.54e-320 &  3.206E-02 &  3.234E-02 \\
\hdashline
24 & PDMP-N4.8e+06 & standard-$\Delta$ & 250 & NA &3.093e-493 & 2.692e-493 & 3.74e-493 & 2.955e-493 & 2.268e-494 &  5.359E-02 &  4.535E-02 \\


==> pdm-ais-v0/batch-aggregated-misc.tex <==
10 & PDMP-N1.0e+05 & cube & 50 & NA & 5.458E+01 &  8.980E-01 & 0 &0 & 4.018E+00 &  7.842E-02 \\
\hdashline
10 & PDMP-N2.0e+05 & cube & 70 & NA & 7.592E+01 &  1.347E+00 & 0 &0 & 1.439E+01 &  1.922E-01 \\
\hdashline
10 & PDMP-N2.0e+05 & cube & 100 & NA & 1.090E+02 &  4.575E+00 & 0 &0 & 2.722E+01 &  9.143E-01 \\
\hline
10 & PDMP-N2.5e+05 & isotropic-$\Delta$ & 50 & NA & 5.314E+01 &  4.235E-01 & 0 &0 & 7.623E+00 &  6.637E-02 \\
\hdashline
10 & PDMP-N7.5e+05 & isotropic-$\Delta$ & 70 & NA & 7.388E+01 &  1.111E+00 & 0 &0 & 3.877E+01 &  3.728E-01 \\
\hdashline
10 & PDMP-N2.0e+06 & isotropic-$\Delta$ & 100 & NA & 1.045E+02 &  1.920E+00 & 0 &0 & 1.865E+02 &  2.508E+00 \\
\hdashline
8 & PDMP-N5.0e+06 & isotropic-$\Delta$ & 250 & NA & 2.603E+02 &  2.079E+00 & 0 &0 & 2.622E+03 &  4.751E+01 \\
\hline
10 & PDMP-N6.0e+05 & standard-$\Delta$ & 50 & NA & 5.273E+01 &  5.523E-01 & 0 &0 & 1.708E+01 &  1.273E-01 \\
\hdashline
10 & PDMP-N8.0e+05 & standard-$\Delta$ & 70 & NA & 7.316E+01 &  6.034E-01 & 0 &0 & 4.021E+01 &  4.736E-01 \\
\hdashline
10 & PDMP-N8.0e+05 & standard-$\Delta$ & 100 & NA & 1.033E+02 &  9.102E-01 & 0 &0 & 7.524E+01 &  1.017E+00 \\
\hdashline
8 & PDMP-N3.5e+06 & standard-$\Delta$ & 250 & NA & 2.573E+02 &  1.367E+00 & 0 &0 & 1.832E+03 &  1.615E+01 \\


==> pdm-ais-v0/batch-aggregated-volumes.tex <==
10 & PDMP-N1.0e+05 & cube & 50 & NA &1.126e+15 & 1.058e+15 & 1.194e+15 & 1.13e+15 & 4.355e+13 &  3.574E-02 &  2.199E-02 \\
\hdashline
10 & PDMP-N2.0e+05 & cube & 70 & NA &1.181e+21 & 1.113e+21 & 1.311e+21 & 1.205e+21 & 5.185e+19 &  3.655E-02 &  3.400E-02 \\
\hdashline
10 & PDMP-N2.0e+05 & cube & 100 & NA &1.268e+30 & 1.196e+30 & 1.331e+30 & 1.253e+30 & 4.413e+28 &  2.871E-02 &  2.147E-02 \\
\hline
10 & PDMP-N2.5e+05 & isotropic-$\Delta$ & 50 & NA &3.421e+21 & 3.226e+21 & 3.662e+21 & 3.512e+21 & 1.471e+20 &  5.167E-02 &  2.364E-02 \\
\hdashline
10 & PDMP-N7.5e+05 & isotropic-$\Delta$ & 70 & NA &1.658e+30 & 1.586e+30 & 1.703e+30 & 1.633e+30 & 3.788e+28 &  1.967E-02 &  1.166E-02 \\
\hdashline
10 & PDMP-N2.0e+06 & isotropic-$\Delta$ & 100 & NA &1.771e+43 & 1.626e+43 & 1.807e+43 & 1.739e+43 & 5.971e+41 &  2.395E-02 &  2.535E-02 \\
\hdashline
8 & PDMP-N5.0e+06 & isotropic-$\Delta$ & 250 & NA &2.466e+108 & 2.284e+108 & 2.739e+108 & 2.48e+108 & 1.347e+107 &  3.041E-02 &  3.698E-02 \\
\hline
10 & PDMP-N6.0e+05 & standard-$\Delta$ & 50 & NA &3.288e-65 & 3.151e-65 & 3.571e-65 & 3.255e-65 & 1.48e-66 &  3.601E-02 &  2.401E-02 \\
\hdashline
10 & PDMP-N8.0e+05 & standard-$\Delta$ & 70 & NA &8.348e-101 & 7.932e-101 & 9.046e-101 & 8.563e-101 & 3.331e-102 &  4.405E-02 &  2.325E-02 \\
\hdashline
10 & PDMP-N8.0e+05 & standard-$\Delta$ & 100 & NA &1.072e-158 & 9.966e-159 & 1.157e-158 & 1.024e-158 & 4.889e-160 &  5.090E-02 &  2.443E-02 \\
\hdashline
8 & PDMP-N3.5e+06 & standard-$\Delta$ & 250 & NA &3.093e-493 & 2.826e-493 & 3.415e-493 & 3.162e-493 & 2.212e-494 &  5.540E-02 &  3.080E-02 \\


==> pdm-ais-v1/batch-aggregated-misc.tex <==
10 & PDMP-N1.0e+05 & cube & 50 & NA & 5.521E+01 &  1.000E+00 & 0 &0 & 4.052E+00 &  8.257E-02 \\
\hdashline
10 & PDMP-N2.0e+05 & cube & 70 & NA & 7.676E+01 &  1.642E+00 & 0 &0 & 1.464E+01 &  3.555E-01 \\
\hdashline
10 & PDMP-N2.0e+05 & cube & 100 & NA & 1.090E+02 &  3.575E+00 & 0 &0 & 2.729E+01 &  4.364E-01 \\
\hline
10 & PDMP-N6.0e+05 & standard-$\Delta$ & 50 & NA & 5.287E+01 &  5.387E-01 & 0 &0 & 1.707E+01 &  1.868E-01 \\
\hdashline
10 & PDMP-N9.0e+05 & standard-$\Delta$ & 70 & NA & 7.326E+01 &  3.571E-01 & 0 &0 & 4.521E+01 &  1.518E+00 \\
\hdashline
10 & PDMP-N1.0e+06 & standard-$\Delta$ & 100 & NA & 1.034E+02 &  7.403E-01 & 0 &0 & 9.318E+01 &  9.664E-01 \\


==> pdm-ais-v1/batch-aggregated-volumes.tex <==
10 & PDMP-N1.0e+05 & cube & 50 & NA &1.126e+15 & 1.071e+15 & 1.185e+15 & 1.125e+15 & 3.386e+13 &  2.697E-02 &  1.820E-02 \\
\hdashline
10 & PDMP-N2.0e+05 & cube & 70 & NA &1.181e+21 & 1.085e+21 & 1.209e+21 & 1.161e+21 & 3.853e+19 &  2.405E-02 &  2.658E-02 \\
\hdashline
10 & PDMP-N2.0e+05 & cube & 100 & NA &1.268e+30 & 1.153e+30 & 1.416e+30 & 1.257e+30 & 8.563e+28 &  3.503E-02 &  4.288E-02 \\
\hline
10 & PDMP-N6.0e+05 & standard-$\Delta$ & 50 & NA &3.288e-65 & 3.147e-65 & 3.464e-65 & 3.342e-65 & 1.106e-66 &  3.834E-02 &  1.912E-02 \\
\hdashline
10 & PDMP-N9.0e+05 & standard-$\Delta$ & 70 & NA &8.348e-101 & 7.798e-101 & 9.095e-101 & 8.52e-101 & 3.657e-102 &  3.486E-02 &  2.585E-02 \\
\hdashline
10 & PDMP-N1.0e+06 & standard-$\Delta$ & 100 & NA &1.072e-158 & 1.005e-158 & 1.2e-158 & 1.063e-158 & 5.758e-160 &  3.384E-02 &  3.468E-02 \\


==> pdm-ais-v2/batch-aggregated-misc.tex <==
50 & PDMP-N1.0e+05 & cube & 50 & NA & 5.468E+01 &  1.501E+00 & 0 &0 & 4.025E+00 &  8.019E-02 \\
\hdashline
10 & PDMP-N1.7e+05 & cube & 70 & NA & 7.657E+01 &  2.232E+00 & 0 &0 & 1.250E+01 &  3.744E-01 \\
\hdashline
10 & PDMP-N1.8e+05 & cube & 100 & NA & 1.096E+02 &  4.416E+00 & 0 &0 & 2.509E+01 &  6.854E-01 \\
\hdashline
10 & PDMP-N3.6e+05 & cube & 140 & NA & 1.524E+02 &  2.518E+00 & 0 &0 & 9.277E+01 &  1.376E+00 \\
\hdashline
10 & PDMP-N8.0e+05 & cube & 175 & NA & 1.931E+02 &  6.807E+00 & 0 &0 & 2.741E+02 &  4.974E+00 \\
\hdashline
10 & PDMP-N1.2e+06 & cube & 250 & NA & 2.674E+02 &  6.395E+00 & 0 &0 & 9.149E+02 &  1.482E+01 \\
\hline
15 & PDMP-N4.0e+05 & isotropic-$\Delta$ & 50 & NA & 5.356E+01 &  3.847E-01 & 0 &0 & 1.180E+01 &  8.601E-01 \\
\hdashline
10 & PDMP-N6.0e+05 & isotropic-$\Delta$ & 70 & NA & 7.405E+01 &  9.160E-01 & 0 &0 & 3.137E+01 &  4.982E-01 \\
\hdashline
10 & PDMP-N1.2e+06 & isotropic-$\Delta$ & 100 & NA & 1.044E+02 &  1.120E+00 & 0 &0 & 1.142E+02 &  1.496E+00 \\
\hdashline
10 & PDMP-N2.4e+06 & isotropic-$\Delta$ & 140 & NA & 1.464E+02 &  2.222E+00 & 0 &0 & 4.342E+02 &  4.457E+00 \\
\hdashline
10 & PDMP-N3.5e+06 & isotropic-$\Delta$ & 175 & NA & 1.850E+02 &  2.136E+00 & 0 &0 & 9.295E+02 &  9.875E+00 \\
\hdashline
10 & PDMP-N6.0e+06 & isotropic-$\Delta$ & 250 & NA & 2.598E+02 &  1.434E+00 & 0 &0 & 3.000E+03 &  3.458E+01 \\
\hline
15 & PDMP-N6.0e+05 & standard-$\Delta$ & 50 & NA & 5.263E+01 &  4.286E-01 & 0 &0 & 1.685E+01 &  1.193E+00 \\
\hdashline
10 & PDMP-N9.0e+05 & standard-$\Delta$ & 70 & NA & 7.328E+01 &  4.673E-01 & 0 &0 & 4.505E+01 &  2.896E-01 \\
\hdashline
50 & PDMP-N1.0e+06 & standard-$\Delta$ & 100 & NA & 1.037E+02 &  6.735E-01 & 0 &0 & 9.465E+01 &  9.332E-01 \\
\hdashline
10 & PDMP-N2.4e+06 & standard-$\Delta$ & 140 & NA & 1.442E+02 &  1.275E+00 & 0 &0 & 3.964E+02 &  1.740E+01 \\
\hdashline
10 & PDMP-N3.5e+06 & standard-$\Delta$ & 175 & NA & 1.795E+02 &  1.051E+00 & 0 &0 & 8.798E+02 &  6.031E+01 \\
\hdashline
10 & PDMP-N5.0e+06 & standard-$\Delta$ & 250 & NA & 2.562E+02 &  1.409E+00 & 0 &0 & 2.356E+03 &  1.465E+02 \\


==> pdm-ais-v2/batch-aggregated-volumes.tex <==
50 & PDMP-N1.0e+05 & cube & 50 & NA &1.126e+15 & 1.048e+15 & 1.218e+15 & 1.114e+15 & 3.989e+13 &  2.731E-02 &  1.931E-02 \\
\hdashline
10 & PDMP-N1.7e+05 & cube & 70 & NA &1.181e+21 & 1.092e+21 & 1.247e+21 & 1.181e+21 & 5.058e+19 &  3.823E-02 &  2.222E-02 \\
\hdashline
10 & PDMP-N1.8e+05 & cube & 100 & NA &1.268e+30 & 1.154e+30 & 1.344e+30 & 1.239e+30 & 5.364e+28 &  3.117E-02 &  2.530E-02 \\
\hdashline
10 & PDMP-N3.6e+05 & cube & 140 & NA &1.394e+42 & 1.263e+42 & 1.443e+42 & 1.377e+42 & 5.119e+40 &  3.106E-02 &  2.567E-02 \\
\hdashline
10 & PDMP-N8.0e+05 & cube & 175 & NA &4.789e+52 & 4.07e+52 & 5.05e+52 & 4.774e+52 & 3.156e+51 &  5.009E-02 &  4.641E-02 \\
\hdashline
10 & PDMP-N1.2e+06 & cube & 250 & NA &1.809e+75 & 1.598e+75 & 1.854e+75 & 1.758e+75 & 8.676e+73 &  3.260E-02 &  3.677E-02 \\
\hline
15 & PDMP-N4.0e+05 & isotropic-$\Delta$ & 50 & NA &3.421e+21 & 3.129e+21 & 3.548e+21 & 3.347e+21 & 9.582e+19 &  3.157E-02 &  2.031E-02 \\
\hdashline
10 & PDMP-N6.0e+05 & isotropic-$\Delta$ & 70 & NA &1.658e+30 & 1.558e+30 & 1.738e+30 & 1.645e+30 & 6.092e+28 &  3.864E-02 &  1.962E-02 \\
\hdashline
10 & PDMP-N1.2e+06 & isotropic-$\Delta$ & 100 & NA &1.771e+43 & 1.624e+43 & 1.903e+43 & 1.807e+43 & 7.723e+41 &  2.650E-02 &  2.692E-02 \\
\hdashline
10 & PDMP-N2.4e+06 & isotropic-$\Delta$ & 140 & NA &4.167e+60 & 3.94e+60 & 4.506e+60 & 4.178e+60 & 1.82e+59 &  3.504E-02 &  2.204E-02 \\
\hdashline
10 & PDMP-N3.5e+06 & isotropic-$\Delta$ & 175 & NA &6.607e+75 & 6.117e+75 & 6.859e+75 & 6.451e+75 & 2.307e+74 &  3.258E-02 &  2.201E-02 \\
\hdashline
10 & PDMP-N6.0e+06 & isotropic-$\Delta$ & 250 & NA &2.466e+108 & 2.261e+108 & 2.624e+108 & 2.471e+108 & 1.169e+107 &  4.736E-02 &  2.820E-02 \\
\hline
15 & PDMP-N6.0e+05 & standard-$\Delta$ & 50 & NA &3.288e-65 & 3.053e-65 & 3.518e-65 & 3.239e-65 & 1.437e-66 &  4.096E-02 &  2.005E-02 \\
\hdashline
10 & PDMP-N9.0e+05 & standard-$\Delta$ & 70 & NA &8.348e-101 & 8.077e-101 & 8.782e-101 & 8.418e-101 & 2.328e-102 &  2.547E-02 &  1.451E-02 \\
\hdashline
50 & PDMP-N1.0e+06 & standard-$\Delta$ & 100 & NA &1.072e-158 & 9.567e-159 & 1.177e-158 & 1.085e-158 & 5.308e-160 &  2.856E-02 &  2.991E-02 \\
\hdashline
10 & PDMP-N2.4e+06 & standard-$\Delta$ & 140 & NA &7.428e-242 & 6.694e-242 & 7.913e-242 & 7.314e-242 & 3.714e-243 &  3.989E-02 &  2.691E-02 \\
\hdashline
10 & PDMP-N3.5e+06 & standard-$\Delta$ & 175 & NA &8.893e-319 & 8.244e-319 & 9.348e-319 & 9.029e-319 & 3.514e-320 &  3.769E-02 &  2.068E-02 \\
\hdashline
10 & PDMP-N5.0e+06 & standard-$\Delta$ & 250 & NA &3.093e-493 & 2.948e-493 & 3.266e-493 & 3.121e-493 & 1.141e-494 &  3.364E-02 &  1.776E-02 \\

